Leveraging Large Language Models to Power Chatbots for Collecting User Self-Reported Data

Large language models (LLMs) provide a new way to build chatbots by accepting natural language prompts. Yet, it is unclear how to design prompts to power chatbots to carry on naturalistic conversations while pursuing a given goal, such as collecting self-report data from users. We explore what design factors of prompts can help steer chatbots to talk naturally and collect data reliably. To this aim, we formulated four prompt designs with different structures and personas. Through an online study (N = 48) where participants conversed with chatbots driven by different designs of prompts, we assessed how prompt designs and conversation topics affected the conversation flows and users' perceptions of chatbots. Our chatbots covered 79% of the desired information slots during conversations, and the designs of prompts and topics significantly influenced the conversation flows and the data collection performance. We discuss the opportunities and challenges of building chatbots with LLMs.

==> sections/99-appendices-backup.tex <==
\section{Appendices}
\subsection{The Web Chatbot Interface}\label{appendix:interface}

\begin{figure}[H]
    \centering
    \includegraphics[width=\textwidth]{img/chat_interface.png}
    \label{fig:web_interface}
    \Description{A screenshot of the web chat interface of GPT-3-based chatbots used in our study. The screen consists of two panels in a horizontal layout. The left panel is a chat interface where participants can see the chatbot's and their messages, and submit a new message. The right panel includes the list of guidelines and instruction. A 'Next' button is located at the bottom of the right panel so that participants can terminate the current conversation and proceed to the next conversation.}
\end{figure}

\subsection{Hint Texts for Conversation Paths}\label{appendix:paths}
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}

The hint texts are displayed in \textcolor[HTML]{1f6adb}{blue} (positive) or \textcolor[HTML]{db411f}{red} (negative) in the instruction (See Appendix \ref{appendix:interface}, right).

\begin{table}[H]
    \small\sffamily
	\def\arraystretch{1.5}\setlength{\tabcolsep}{0.5em}
		    \flushleft
\begin{tabular}{|l|l!{\color{lightgray}\vrule}l|}
\hline
\rowcolor{tableheader} & \textbf{Positive Path}                               & \textbf{Negative Path}                             \\ \hline
\textbf{Sleep}    & You had \textit{\textbf{good sleep}} last night.     & You had \textbf{\textit{bad sleep}} last night.   \\ \arrayrulecolor{tablegrayline}\hline
\textbf{Work}     & You were \textit{\textbf{productive}} yesterday.     & You \textit{\textbf{did nothing}} yesterday.      \\ \hline
\textbf{Food Intake}     & You \textit{\textbf{had all three meals}} yesterday. & You \textit{\textbf{skipped one meal}} yesterday. \\ \hline
\textbf{Exercise} & You \textit{\textbf{exercised}} yesterday.           & You \textit{\textbf{did not exercise}} yesterday. \\ \arrayrulecolor{black}\hline
\end{tabular}%
\label{tab:hints}
\end{table}

\newpage
\subsection{Least-Squared Mean Statistics for Slot Filling Rate}

Estimation based on a significant linear model formula:
\newline
$SlotFillingRate = Personality+Format+Topic+Path+Personality \times Format$
\newline
$F(7,366)=6.493, p<.0001$***

\begin{table}[H]
\small\sffamily
	\def\arraystretch{1.2}\setlength{\tabcolsep}{0.5em}
\centering
\caption{Estimated least-squared means with 95\% confidence intervals (CI) of slot filling rate by condition.}
\begin{tabular}{|l|lllll|}
\hline
\rowcolor{tableheader} \textbf{Condition} & \textbf{Est. Mean}     & \textbf{\textit{SE}}         & \textbf{df}  & \textbf{Lower CI}   & \textbf{Upper CI}    \\
\hline
\textbf{SP}        & 83.03\% & 2.60 & 366 & 77.91 & 88.16  \\ \arrayrulecolor{tablegrayline}\hline
\textbf{SN}        & 75.99\% & 2.54 & 366 & 71.00 & 80.98  \\ \hline
\textbf{DP}        & 71.90\% & 2.55 & 366 & 66.89 & 76.91  \\ \hline
\textbf{DN}        & 83.43\% & 2.59 & 366 & 78.33 & 88.52 \\
\arrayrulecolor{black}\hline
\end{tabular}
\end{table}


\begin{table}[H]
\small\sffamily
	\def\arraystretch{1.2}\setlength{\tabcolsep}{0.5em}
\centering
\caption{Estimated least-squared means with 95\% confidence intervals (CI) of slot filling rate by topic.}
\begin{tabular}{|l|lllll|}
\hline
\rowcolor{tableheader} \textbf{Topic} & \textbf{Est. Mean}     & \textbf{\textit{SE}}         & \textbf{df}  & \textbf{Lower CI}   & \textbf{Upper CI}    \\
\hline
\textbf{Sleep}    & 77.35\% & 2.56 & 366 & 72.31 & 82.39  \\ \arrayrulecolor{tablegrayline}\hline
\textbf{Work}     & 70.69\% & 2.61 & 366 & 65.57 & 75.81  \\ \hline
\textbf{Food}     & 77.91\% & 2.55 & 366 & 72.89 & 82.92  \\ \hline
\textbf{Exercise} & 88.40\% & 2.56 & 366 & 83.36 & 93.44  \\ \arrayrulecolor{black} \hline
\end{tabular}
\end{table}


\begin{table}[H]
\small\sffamily
	\def\arraystretch{1.2}\setlength{\tabcolsep}{0.5em}
\centering
\caption{Estimated least-squared means with 95\% confidence intervals (CI) of slot filling rate by conversation path.}
\begin{tabular}{|l|lllll|}
\hline
\rowcolor{tableheader} \textbf{Path} & \textbf{Est. Mean}     & \textbf{\textit{SE}}         & \textbf{df}  & \textbf{Lower CI}   & \textbf{Upper CI}    \\
\hline
\textbf{Positive} & 81.88\% & 1.82 & 366 & 78.31 & 85.45  \\ \arrayrulecolor{tablegrayline}\hline
\textbf{Negative} & 75.30\% & 1.82 & 366 & 71.72 & 78.87  \\\arrayrulecolor{black} \hline
\end{tabular}
\end{table}


\iffalse
\begin{table}[H]
\small\sffamily
	\def\arraystretch{1.2}\setlength{\tabcolsep}{0.5em}
\centering
\caption{Estimated least-squared means with 95\% confidence intervals (CI) of slot filling rate by condition.}
\begin{tabular}{|l|lllll|}
\hline
\rowcolor{tableheader}
\textbf{Contrast} & \textbf{Effect size} & \textbf{\textit{SE}} & \textbf{df} & \textbf{\textit{t}-statistic} & \textbf{\textit{p}-value}  \\ \hline
\textbf{DN - DP}  & 11.53           & 3.63  & 366         & 3.17           & 0.00888172        \\ \arrayrulecolor{tablegrayline}\hline
\textbf{DN - SN}  & 7.44            & 3.62   & 366         & 2.05           & 0.17105564        \\ \hline
\textbf{DN - SP}  & 0.39           & 3.67  & 366         & 0.11            & 0.99955672        \\ \hline
\textbf{DP - SN}  & -4.09            & 3.60  & 366         & -1.14           & 0.66648961        \\ \hline
\textbf{DP - SP}  & -11.13           & 3.64  & 366         & -3.06            & 0.0128534         \\ \hline
\textbf{SN - SP}  & -7.04           & 3.64  & 366         & -1.94           & 0.21405601       \\ \arrayrulecolor{black}
\hline
\end{tabular}
\end{table}
\fi

\subsection{Least-Squared Mean Statistics for Required and Secondary Question Turn Ratios}
\subsubsection{Turn Ratio of Required Questions}
Estimation based on a mixed-effect model fitted:
\newline
$RQTurnRatio = Personality+Format+Topic+Path+Personality \times Format + Topic \times Path$
\newline
with significant random effect of participants ($p<.0001$***)


\begin{table}[H]
\small\sffamily
	\def\arraystretch{1.2}\setlength{\tabcolsep}{0.5em}
\centering
\caption{Estimated least-squared means with 95\% confidence intervals (CI) of RQ turn ratio by information format.}
\begin{tabular}{|l|lllll|}
\hline
\rowcolor{tableheader} \textbf{Format} & \textbf{Est. Mean}     & \textbf{\textit{SE}}         & \textbf{df}  & \textbf{Lower CI}   & \textbf{Upper CI}    \\
\hline
\textbf{Specific}    & 22.44\%  & 1.03 & 43.99 & 20.36 & 24.51  \\ \arrayrulecolor{tablegrayline}\hline
\textbf{Descriptive} & 19.21\% & 1.03 & 43.97  & 17.14 & 21.29   \\\arrayrulecolor{black} \hline
\end{tabular}
\end{table}


\begin{table}[H]
\small\sffamily
\def\arraystretch{1.2}\setlength{\tabcolsep}{0.5em}
\centering
\caption{Estimated least-squared means with 95\% confidence intervals (CI) of RQ turn ratio by condition.}
\begin{tabular}{|l|lllll|}
\hline
\rowcolor{tableheader} \textbf{Condition} & \textbf{Est. Mean}     & \textbf{\textit{SE}}         & \textbf{df}  & \textbf{Lower CI}   & \textbf{Upper CI}    \\
\hline
\textbf{SP} & 23.93\% & 1.47 & 44.94  & 20.98 & 26.88  \\ \arrayrulecolor{tablegrayline}\hline
\textbf{SN} & 20.94\% & 1.45 & 43.05 & 18.02 & 23.86  \\ \hline
\textbf{DP} & 17.63\% & 1.45 & 43.41 & 14.70  & 20.56  \\ \hline
\textbf{DN} & 20.80\% & 1.46 & 44.54 & 17.85 & 23.74 \\\arrayrulecolor{black} \hline
\end{tabular}
\end{table}


\begin{table}[H]
\small\sffamily
	\def\arraystretch{1.2}\setlength{\tabcolsep}{0.5em}
\centering
\caption{Estimated least-squared means with 95\% confidence intervals (CI) of RQ turn ratio by conversation path.}
\begin{tabular}{|l|lllll|}
\hline
\rowcolor{tableheader} \textbf{Path} & \textbf{Est. Mean}     & \textbf{\textit{SE}}         & \textbf{df}  & \textbf{Lower CI}   & \textbf{Upper CI}    \\
\hline
\textbf{Positive} & 21.92\% & 0.86 & 82.65 & 20.22 & 23.63  \\ \arrayrulecolor{tablegrayline}\hline
\textbf{Negative} & 19.73\% & 0.86 & 82.53 & 18.02 & 21.43  \\\arrayrulecolor{black} \hline
\end{tabular}
\end{table}


\begin{table}[H]
\small\sffamily
	\def\arraystretch{1.2}\setlength{\tabcolsep}{0.5em}
\centering
\caption{Estimated least-squared means with 95\% confidence intervals (CI) of RQ turn ratio by topic and conversation path.}
\begin{tabular}{|ll|lllll|}
\hline
\rowcolor{tableheader} \textbf{Topic} & \textbf{Path} & \textbf{Est. Mean}     & \textbf{\textit{SE}}         & \textbf{df}  & \textbf{Lower CI}   & \textbf{Upper CI}    \\
\hline
\multirow{2}{*}{\textbf{Sleep}}    & \textbf{Positive} & 22.73\% & 1.38  & 295.42 & 20.01 & 25.45  \\
\arrayrulecolor{tablegrayline}\cline{2-7}
    & \textbf{Negative} & 23.78\% & 1.41 & 301.42 & 21.00 & 26.55   \\
\arrayrulecolor{gray}\hline
\multirow{2}{*}{\textbf{Work}}     & \textbf{Positive} & 19.13\% & 1.44 & 307.50 & 16.30  & 21.96  \\
\arrayrulecolor{tablegrayline}\cline{2-7}
     & \textbf{Negative} & 15.04\% & 1.40 & 298.34 & 12.29 & 17.78  \\
\arrayrulecolor{gray}\hline
\multirow{2}{*}{\textbf{Food}}    & \textbf{Positive} & 24.03\% & 1.38  & 295.42 & 21.31 & 26.75  \\
\arrayrulecolor{tablegrayline}\cline{2-7}
     & \textbf{Negative} & 23.54\% & 1.40 & 298.34 & 20.79 & 26.28  \\
\arrayrulecolor{gray}\hline
\multirow{2}{*}{\textbf{Exercise}} & \textbf{Positive} & 21.81\% & 1.40 & 298.44 & 19.06  & 24.56  \\
\arrayrulecolor{tablegrayline}\cline{2-7}
 & \textbf{Negative} & 16.55\% & 1.40 & 298.44 & 13.81 & 19.30 \\
\arrayrulecolor{black} \hline
\end{tabular}
\vspace{5mm}
\end{table}


\subsubsection{Turn Ratio of Secondary Questions}
Estimation based on a significant linear model formula:
\newline
$SQTurnRatio = Personality+Format+Topic+Path + Topic \times Path$
\newline
$F(9,364)=10.04, p<.0001$***



\begin{table}[H]
\small\sffamily
	\def\arraystretch{1.2}\setlength{\tabcolsep}{0.5em}
\centering
\caption{Estimated least-squared means with 95\% confidence intervals (CI) of SQ turn ratio by information format.}
\begin{tabular}{|l|lllll|}
\hline
\rowcolor{tableheader} \textbf{Format} & \textbf{Est. Mean}     & \textbf{\textit{SE}}         & \textbf{df}  & \textbf{Lower CI}   & \textbf{Upper CI}    \\
\hline
\textbf{Specific}    & 9.64\%  & 0.68 & 364 & 8.30 & 10.97  \\ \arrayrulecolor{tablegrayline}\hline
\textbf{Descriptive} & 12.55\% & 0.68 & 364  & 11.22 & 13.88   \\\arrayrulecolor{black} \hline
\end{tabular}
\end{table}


\begin{table}[H]
\small\sffamily
\def\arraystretch{1.2}\setlength{\tabcolsep}{0.5em}
\centering
\caption{Estimated least-squared means with 95\% confidence intervals (CI) of SQ turn ratio by condition.}
\begin{tabular}{|l|lllll|}
\hline
\rowcolor{tableheader} \textbf{Condition} & \textbf{Est. Mean}     & \textbf{\textit{SE}}         & \textbf{df}  & \textbf{Lower CI}   & \textbf{Upper CI}    \\
\hline
\textbf{SP} & 9.26\% & 0.84 & 364  & 7.62 & 10.91  \\ \arrayrulecolor{tablegrayline}\hline
\textbf{SN} & 10.01\% & 0.82 & 364 & 8.40 & 11.63  \\ \hline
\textbf{DP} & 12.18\% & 0.82 & 364 & 10.56  & 13.80  \\ \hline
\textbf{DN} & 12.93\% & 0.83 & 364 & 11.29 & 14.57 \\\arrayrulecolor{black} \hline
\end{tabular}
\end{table}


\begin{table}[H]
\small\sffamily
	\def\arraystretch{1.2}\setlength{\tabcolsep}{0.5em}
\centering
\caption{Estimated least-squared means with 95\% confidence intervals (CI) of RQ turn ratio by conversation path.}
\begin{tabular}{|l|lllll|}
\hline
\rowcolor{tableheader} \textbf{Path} & \textbf{Est. Mean}     & \textbf{\textit{SE}}         & \textbf{df}  & \textbf{Lower CI}   & \textbf{Upper CI}    \\
\hline
\textbf{Positive} & 9.59\% & 0.68 & 364 & 8.26 & 10.92  \\ \arrayrulecolor{tablegrayline}\hline
\textbf{Negative} & 12.60\% & 0.68 & 364 & 11.27 & 13.93  \\\arrayrulecolor{black} \hline
\end{tabular}
\end{table}


\begin{table}[H]
\small\sffamily
	\def\arraystretch{1.2}\setlength{\tabcolsep}{0.5em}
\centering
\caption{Estimated least-squared means with 95\% confidence intervals (CI) of SQ turn ratio by topic and conversation path.}
\begin{tabular}{|ll|lllll|}
\hline
\rowcolor{tableheader} \textbf{Topic} & \textbf{Path} & \textbf{Est. Mean}     & \textbf{\textit{SE}}         & \textbf{df}  & \textbf{Lower CI}   & \textbf{Upper CI}    \\
\hline
\multirow{2}{*}{\textbf{Sleep}}    & \textbf{Positive} & 7.71\% & 1.34  & 364 & 5.08 & 10.33  \\
\arrayrulecolor{tablegrayline}\cline{2-7}
    & \textbf{Negative} & 7.17\% & 1.36 & 364 & 4.49 & 9.85   \\
\arrayrulecolor{gray}\hline
\multirow{2}{*}{\textbf{Work}}     & \textbf{Positive} & 14.23\% & 1.39 & 364 & 11.49  & 16.98  \\
\arrayrulecolor{tablegrayline}\cline{2-7}
     & \textbf{Negative} & 20.03\% & 1.35 & 364 & 17.38 & 22.68  \\
\arrayrulecolor{gray}\hline
\multirow{2}{*}{\textbf{Food}}    & \textbf{Positive} & 9.66\% & 1.34  & 364 & 7.04 & 12.29  \\
\arrayrulecolor{tablegrayline}\cline{2-7}
     & \textbf{Negative} & 9.48\% & 1.35 & 364 & 6.83 & 12.13  \\
\arrayrulecolor{gray}\hline
\multirow{2}{*}{\textbf{Exercise}} & \textbf{Positive} & 6.76\% & 1.35 & 364 & 4.11  & 9.42  \\
\arrayrulecolor{tablegrayline}\cline{2-7}
 & \textbf{Negative} & 13.70\% & 1.35 & 364 & 11.05 & 16.35 \\
\arrayrulecolor{black} \hline
\end{tabular}
\vspace{5mm}
\end{table}


\subsection{Least-Squared Mean Statistics for Chatbot Behavioral Turn Ratios}

\subsubsection{Chatbot's Acknowledging Turn Ratio}

==> tables/dialogue-acts.tex <==
% Please add the following required packages to your document preamble:
% 

\begin{table}[b]
    \small\sffamily
	\def\arraystretch{1.2}\setlength{\tabcolsep}{0.25em}
		    \centering
\caption{Summary of dialogue acts with brief description and exemplar turns (\symboluser{}: user turns, \symbolbot{}: chatbot turns).}
\label{tab:dialogue_acts}
\begin{tabular}{|p{0.19\textwidth}|p{0.32\textwidth}!{\color{lightgray}\vrule}p{0.45\textwidth}|}
\hline
\rowcolor{tableheader}
 \textbf{Dialogue Act} &
  \textbf{Description} &
  \textbf{Example} \\ 
  
  \rowcolor{darkgray}\multicolumn{3}{|l|}{\textcolor{white}{Essential Acts}} \\
  
\textbf{Greeting} & Initiation of a conversation. &
  \parbox[t]{0.45\textwidth}{\symbolbot{} \textit{How's your day so far?}\\ \symboluser{} \textit{I feel refreshed and recharged.}\vspace{0.5mm}} \\
  \arrayrulecolor{tablegrayline}\hline
  
  \textbf{Task opening} & \parbox[t]{0.30\textwidth}{General questions that bring up\\the conversation topic.\vspace{0.5mm}} &
  \symbolbot{} \textit{How was your work and productivity yesterday?} \\\hline
  \parbox[t]{0.20\textwidth}{\textbf{Required}\\\textbf{questions/answers}} & \parbox[t]{0.30\textwidth}{Q\&As that are directly related to\\the specified information slots.\vspace{0.5mm}}  &
  \parbox[t]{0.45\textwidth}{\symbolbot{} \textit{What was your lunch yesterday?} (RQ)\\ \symboluser{} \textit{I had pork barbeque.} (RA)\vspace{0.5mm}} \\ \hline
 \parbox[t]{0.20\textwidth}{\textbf{Secondary}\\\textbf{questions/answers}} & \parbox[t]{0.30\textwidth}{Q\&As that are usually follow-ups and\\not specific to the information slots.\vspace{0.5mm}} &
  \parbox[t]{0.45\textwidth}{\symbolbot{} \textit{What did you put on your toast?} (SQ)\\ \symboluser{} \textit{I put strawberry jam on it.} (SA)\vspace{0.5mm}} \\ \hline
  
  \textbf{Statement} & \parbox[t]{0.30\textwidth}{Non-Q\&A messages such as\\commenting or summarizing.\vspace{0.5mm}} &
  \parbox[t]{0.45\textwidth}{\symbolbot{} \textit{It sounds like you had a great night's sleep!}\\ \symboluser{} \textit{I did! Not sure why though.}\vspace{0.5mm}} \\\hline
  
  \textbf{Closing} & Farewell or ending messages. &
  \symbolbot{} You're welcome. Have a great day! \\ 
\arrayrulecolor{black}  
\rowcolor{darkgray}\multicolumn{3}{|l|}{\textcolor{white}{Empathy \& Engagement Behaviors}} \\
  
\textbf{Acknowledging} & Directly referring to what the other said. &
  \symbolbot{} \textit{That's great to hear that your legs are feeling stronger!} \\\arrayrulecolor{tablegrayline}\hline
  
\textbf{Appreciating} & Complimenting the other. &
  \symbolbot{} \textit{That's terrific!} \\ \hline
\textbf{Thanking} & Being grateful to the other. &
  \symboluser{} \textit{I feel nice. Thanks for asking.} \\\hline
  
\textbf{Sympathizing} & Expressing sympathy for the other. &
  \symbolbot{} \textit{I'm sorry to hear that. What's been going on?} \\ \hline
\textbf{Advice/suggesting} & Giving advice or suggestion. &
  \begin{tabular}{@{}l@{}l@{}}\symbolbot{} & \parbox[t]{0.45\textwidth}{ \textit{I can give you some recommendations on exercises that\\will help you grow your adductor muscles.}}\end{tabular} \\\hline
  
\textbf{Rejecting/disagreeing} & Rejecting or disagreeing with the other. &
  \symboluser{} \textit{But the weather needs to be good for walking.} \\
  \arrayrulecolor{black}\hline
\end{tabular}
\end{table}

==> tables/essential_breakdown.tex <==
\begin{table}[t]
    \small\sffamily
	\def\arraystretch{1.2}\setlength{\tabcolsep}{1em}
		    \centering
\caption{The essential component breakdown of dialogues under each condition. The values are expressed in percentages (\%).}
\label{tab:essential_components}
\begin{tabular}{|l|c!{\color{lightgray}\vrule}c!{\color{lightgray}\vrule}c!{\color{lightgray}\vrule}c|}
\hline
\rowcolor{tableheader}\textbf{Essential Acts}              & \textbf{SP}             & \textbf{SN}             & \textbf{DP}             & \textbf{DN}             \\ \hline
\textbf{Greeting}      & 11.17          & 10.01          & 9.43           & 9.06           \\ \arrayrulecolor{tablegrayline}\hline
\textbf{Topic opening} & 1.65           & 1.38           & 0.41           & 0.05           \\ \hline
\textbf{RQ}           & \textbf{23.26} & \textbf{19.49} & \textbf{16.59} & \textbf{19.7}  \\ \hline
\textbf{RA}           & 22.89          & 19.01          & 16.49          & 19.7           \\ \hline
\textbf{SQ}            & \textbf{11.66} & \textbf{13.03} & \textbf{14.58} & \textbf{15.65} \\ \hline
\textbf{SA}            & 10.44          & 11.92          & 13.81          & 14.33          \\ \hline
\textbf{Statement}     & 15.32          & 21.24          & 24.99          & 17.87          \\ \hline
\textbf{Closing}       & 3.6            & 3.92           & 3.71           & 3.65           \\ \arrayrulecolor{black}\hline
\end{tabular}
\end{table}
